The Inverse-Wisdom Law: Architectural Tribalism and the Consensus Paradox in Agentic Swarms

As AI transitions toward multi-agent systems (MAS) to solve complex workflows, research paradigms operate on the axiomatic assumption that agent collaboration mirrors the "Wisdom of the Crowd". We challenge this assumption by formalizing the Consensus Paradox: a phenomenon where agentic swarms prioritize internal architectural agreement over external logical truth. Through a 36 experiments encompassing 12,804 trajectories across three state-of-the-art (SOTA) benchmarks (GAIA, Multi-Challenge, and SWE-bench), we prove the Inverse-Wisdom Law: in kinship-dominant swarms, adding logical agents increases the stability of erroneous trajectories rather than the probability of truth. The introduction of additional logical audits converges the system toward a Logic Saturation where internal entropy hits zero while factual error hits unity. By evaluating the interaction between the 3 preeminent SOTA models (Gemini 3.1 Pro, Claude Sonnet 4.6, and GPT-5.4), we establish the Architectural Tribalism Asymmetry as a mechanistic law of transformer weights. We demonstrate that terminal swarm integrity is strictly gated by the synthesizer's receptive logic, rather than aggregate agent quality. We define the Tribalism Coefficient and the Sycophantic Weight as the primary mechanistic determinants of swarm failure. Finally, we establish the Heterogeneity Mandate as a foundational safety requirement for resilient agentic architectures.

==> checklist.tex <==
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract and introduction accurately reflect the paper's contributions by explicitly defining the formalization of the \textit{Consensus Paradox} and the derivation of the \textit{Inverse-Wisdom Law} as the primary theoretical outcomes. The scope of the investigation is clearly delineated, encompassing a comprehensive audit of \textbf{12,804 trajectories} conducted across three state-of-the-art benchmarks (\textbf{GAIA, Multi-Challenge, and SWE-bench}) using three preeminent model families (\textbf{Gemini, Claude, and GPT-5.4}). Furthermore, the introduction provides a structured list of 7 primary technical contributions, ranging from the \textit{Synthesizer Gating Theorem} to the \textit{Heterogeneity Mandate}, ensuring that the claims match the theoretical and experimental results detailed in the subsequent sections.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper includes a dedicated section (Section 5) that identifies four primary technical boundaries to the current formalism. (1) \textbf{Scaling Limits:} Our validation is grounded in $n=3$ agentic decision chains, and while generalized via induction, emergent properties in massive swarms ($n > 100$) remain an open research question. (2) \textbf{Cross-Modal Generalization:} The \textit{Inverse-Wisdom Law} is currently established for text-based reasoning; future work must verify if cross-modal kinship (e.g., Vision/Audio) triggers the same \textit{Attention Latch} mechanics. (3) \textbf{System Framing:} We held system prompts constant to isolate architectural bias; thus, the specific role of ``Authority'' in breaking the tribal gating mechanism has not been fully isolated. (4) \textbf{Metacognitive Scaffolding:} The work identifies the necessity of \textbf{Stalemate Filtering} based on high-entropy states ($H_2$) but does not implement this mitigation within the current interaction matrix.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper establishes a formal axiomatic foundation in Section 2, defining the state space, agent roles, and the four primary gating parameters ($B, \tau, \sigma, \Lambda$). Every theoretical result presented in the main body (Theorems 1--4) with Lemmas and corollaries is accompanied by a formal derivation. To ensure mathematical rigor, the complete, step-by-step proofs derived from first principles are provided in the Appendix, including the stochastic derivation of the \textit{Attention Latch Factor}, Architectural distance, The Architectural Tribalism Asymmetry, the non-linear coupling of the \textit{Logic Saturation}, and the \textit{Sycophantic Scaling Law}. All theorems, lemmas, and corollaries are uniquely numbered and cross-referenced to maintain structural clarity.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper provides a comprehensive procedural roadmap of the \textbf{Heuristic Taint-Tracking Protocol} in Section 3. We disclose the functional roles and standardized prompt templates for the \textit{Propagator}, \textit{Auditor}, and \textit{Synthesizer} nodes, including the specific domain-aligned \textit{Taint IDs} and ``sleeper instructions'' used to measure error propagation across all 36 interaction arms. The scale of the audit is clearly defined ($N=12,804$ trajectories), encompassing specific model families (\textbf{Gemini, Claude, and GPT-5.4}) with Temperature 0 and three open source benchmark datasets (\textbf{GAIA, Multi-Challenge, and SWE-bench}). Furthermore, we explicitly document the use of held-out \textbf{Test Data Splits} and our deterministic evaluation heuristics to ensure that the reported \textit{True Cascade Rates} and mechanistic coefficients are reproducible on novel logical states.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: While the paper provides a complete procedural roadmap of the \textbf{Heuristic Taint-Tracking Protocol} and the standardized prompt templates required for reproduction in Section 3, the specific implementation code and internal data logs are not currently open-access. Access to the full code repository and raw trajectory datasets will be provided to researchers upon approval. We note that the benchmarks utilized in this study (\textbf{GAIA, Multi-Challenge, and SWE-bench}) are publicly available, and the model families (\textbf{Gemini, Claude, and GPT-5.4}) are accessible via standard API interfaces, enabling independent verification of the \textit{Architectural Tribalism Asymmetry} using the disclosed methodology.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3 detailed the experimental setup, including the selection of the three benchmark datasets (\textbf{GAIA, Multi-Challenge, and SWE-bench}) and the three preeminent model families (\textbf{Gemini, Claude, and GPT-5.4}) under investigation. We explicitly documented the use of held-out \textbf{Test Data Splits} to ensure zero-shot reasoning fidelity and to isolate architectural interaction dynamics from memorized distributions. The functional roles of the \textit{Propagator}, \textit{Auditor}, and \textit{Synthesizer} are defined, and system prompts were held constant to isolate the mechanistic interaction between transformer weights. Specific sample sizes ($N$) for each benchmark and interaction arm are provided to ensure statistical robustness and to parameterize the \textit{Inverse-Wisdom Law} derived in Section 2.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper reports 95\% Confidence Intervals (CI) for all primary outcome metrics, including the \textit{True Cascade Rate} ($\mu$), \textit{Critic Accuracy} ($B$), \textit{Tribalism Coefficient} ($\tau$), and \textit{Sycophantic Weight} ($\sigma$). These measures are explicitly documented in Table 2 and visualized across all 36 interaction arms in Figure 2. Error bars are derived from the \textbf{standard error of the empirical probabilities} across \textbf{12,804 trajectories}, using the standard closed-form formula for binomial proportions. The factors of variability captured include the cross-domain distribution across Multi-Challenge ($N=266$ per arm), GAIA ($N=301$ per arm), and SWE-bench ($N=500$ per arm). We assume normally distributed errors for the large-sample estimators provided by our 12,804-trajectory audit, ensuring that the deltas observed in the \textit{Architectural Tribalism Asymmetry} are statistically definitive.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments were conducted using Open API Keys for the three SOTA model families (Gemini 3.1 Pro, Claude Sonnet 4.6, and GPT-5.4) and standard CPU-based compute workers for the Heuristic Taint-Tracking Protocol and evaluation. We executed a total of 12,804 trajectories, with computational efficiency optimized through the use of robust regex parsing and heuristic refusal filters to verify terminal outcomes. As disclosed in Section 3.6, we performed preliminary validation experiments comparing this heuristic approach to \textit{LLM-as-a-Judge} (using Gemini 2.5 Flash), concluding that our method provided identical accuracy without the associated model-based inference overhead, thereby enabling the scale required for this high-resolution audit.

    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The research conducted in this paper conforms to the NeurIPS Code of Ethics by identifying and formalizing critical interactional failure modes that pose fundamental risks to the integrity of autonomous systems. Our investigation of \textbf{12,804 trajectories} is a controlled, diagnostic audit designed to improve the safety and reliability of agentic swarms, establishing the \textit{Heterogeneity Mandate} as a primary design constraint for achieving \textbf{L5-level autonomous governance}. The work did not involve human subjects, and all evaluations were performed on publicly available benchmarks using standard API access to state-of-the-art models. By uncovering the mechanistic drive to reduce group entropy over factual truth, this study provides a foundational technical framework to prevent \textit{Hallucination Cascades} and ensure the ethical deployment of large-scale agentic systems.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper discusses positive societal impacts by providing a foundational technical framework to prevent \textit{Hallucination Cascades} and improve the reliability of autonomous systems. We explicitly identify the \textit{Heterogeneity Mandate} as a primary design constraint for achieving L5-level autonomous governance. Potential negative impacts are addressed by characterizing the \textit{Consensus Paradox} and the \textit{Inverse-Wisdom Law} as physical risks to truth if current architectural alignment biases remain unmitigated. The work proposes specific mitigation strategies, including architectural diversification and the implementation of \textit{Stalemate Filtering}, to ensure the ethical and safe deployment of large-scale agentic swarms.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work does not release new pre-trained models or high-risk datasets; all evaluations were performed on publicly available benchmarks using standard API access to established state-of-the-art model families (Gemini, Claude, and GPT-5.4). Our investigation is a controlled, diagnostic audit of 12,804 trajectories specifically designed to uncover interactional failure modes and provide the technical foundation for the \textit{Heterogeneity Mandate}. The proposed mitigation strategies, including the \textit{Resilience Inequality} and \textit{Stalemate Filtering}, serve as the primary safeguards for ensuring the ethical and reliable deployment of large-scale agentic systems in the transition toward L5-level autonomous governance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: All existing assets utilized in this study are properly credited through citations of their original publications. Specifically, we use the \textbf{GAIA} benchmark, the \textbf{SWE-bench} repository, and the \textbf{Multi-Challenge} dataset. Evaluation was conducted via standard API access to state-of-the-art model families: \textbf{Gemini 3.1 Pro} (Google), \textbf{Claude Sonnet 4.6} (Anthropic), and \textbf{GPT-5.4} (OpenAI). All model usage adheres to the respective providers' Terms of Service and API usage guidelines, and we confirm that no proprietary model weights or internal datasets were released. Versions and URLs for all assets are provided in the Experimental Methodology (Section 3). 
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This work does not introduce or release new public software assets, general-purpose datasets, or pre-trained models. The primary contributions of the paper are the formal mechanistic theory of the \textit{Consensus Paradox} and the associated interactive interaction laws derived from our large-scale audit. All empirical evaluations were conducted on established, publicly available benchmarks (\textbf{GAIA, Multi-Challenge, and SWE-bench}) using standard API access to existing model families. While the paper describes and parameterizes a comprehensive interaction matrix of \textbf{12,804 trajectories}, this dataset serves as the empirical validation for our theoretical proofs rather than a newly released standalone asset for the community.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This study did not involve crowdsourcing experiments or research with human subjects. All empirical evaluations were conducted on established, publicly available benchmarks (\textbf{GAIA, Multi-Challenge, and SWE-bench}) using standard API access to existing large language model families: \textbf{Gemini, Claude, and GPT-5.4}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: This study did not involve crowdsourcing experiments or research with human subjects. All empirical evaluations were conducted on established, publicly available benchmarks (\textbf{GAIA, Multi-Challenge, and SWE-bench}) using standard API access to existing large language model families: \textbf{Gemini, Claude, and GPT-5.4}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: LLMs are the fundamental components of the core methodology, serving as the functional agents (\textit{Propagator}, \textit{Auditor}, and \textit{Synthesizer}) within the multi-agent swarms under investigation. The research identifies and formalizes the \textit{Consensus Paradox} by systematically evaluating the interaction dynamics between these model families across \textbf{12,804 trajectories}. Additionally, as disclosed in Section 3.6, an LLM (\textbf{Gemini 2.5 Flash}) was utilized as a baseline judge to validate our deterministic evaluation protocol, ensuring that the heuristic verification mechanism matched the accuracy of model-based judgment. LLMs were also used for theorems and proofs verification and enhancement and code debugging.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}
